Adversarial Generative Flow Network for Solving Vehicle Routing Problems

Recent research into solving vehicle routing problems (VRPs) has gained significant traction, particularly through the application of deep (reinforcement) learning for end-to-end solution construction. However, many current construction-based neural solvers predominantly utilize Transformer architectures, which can face scalability challenges and struggle to produce diverse solutions. To address these limitations, we introduce a novel framework beyond Transformer-based approaches, i.e., Adversarial Generative Flow Networks (AGFN). This framework integrates the generative flow network (GFlowNet)-a probabilistic model inherently adept at generating diverse solutions (routes)-with a complementary model for discriminating (or evaluating) the solutions. These models are trained alternately in an adversarial manner to improve the overall solution quality, followed by a proposed hybrid decoding method to construct the solution. We apply the AGFN framework to solve the capacitated vehicle routing problem (CVRP) and travelling salesman problem (TSP), and our experimental results demonstrate that AGFN surpasses the popular construction-based neural solvers, showcasing strong generalization capabilities on synthetic and real-world benchmark instances.

==> Table/1000_nodes.tex <==
\begin{table*}[t!] \color{blue}
    \centering
    \caption{\textcolor{blue}{Comparative results on synthetic CVRP and TSP dataset with 10,000 nodes.}}
    \label{Table: Larger_instances_10000}
    \begin{tabular}{c c c c}
    \toprule \toprule
    \textbf{AGFN-100} & \textbf{Obj.} & \textbf{Gap (\%)} & \textbf{Time (s)} \\
    \midrule
    CVRP & 1146.165161 & - & 14.60 \\
    TSP & 143.848511 & 89.83 & 14.07 \\
    \bottomrule \bottomrule
    \end{tabular}
\end{table*}
